Observation of Time Reversal Violation in the B0 Meson System

Although CP violation in the B meson system has been well established by the B factories, there has been no direct observation of time reversal violation. The decays of entangled neutral B mesons into definite flavor states ($B^0$ or $\bar{B}^0$), and $J/\psi K_S^0$ or $c\bar{c} K_S^0$ final states (referred to as $B_+$ or $B_-$), allow comparisons between the probabilities of four pairs of T-conjugated transitions, for example, $\bar{B}^0 \rightarrow B_-$ and $B_- \rightarrow \bar{B}^0$, as a function of the time difference between the two B decays. Using 468 million $B\bar{B}$ pairs produced in $\Upsilon(4S)$ decays collected by the BABAR detector at SLAC, we measure T-violating parameters in the time evolution of neutral B mesons, yielding $\Delta S_T^+ = -1.37 \pm 0.14 (stat.) \pm 0.06 (syst.)$ and $\Delta S_T^- = 1.17 \pm 0.18 (stat.) \pm 0.11 (syst.)$. These nonzero results represent the first direct observation of T violation through the exchange of initial and final states in transitions that can only be connected by a T-symmetry transformation.

==> babarsym.tex <==
 
\RequirePackage{xspace} 
 
 
% Huge boldface 
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}} 
% LARGE 
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}} 
% Large 
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}} 
% normal size 
% replace normalsize with scalable version       dbm 7/4/00 
\usepackage{relsize} 
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em 
    B\kern-0.1em{\smaller A\kern-0.2em R}}} 
 
\let\emi\en 
\def\electron   {\ensuremath{e}\xspace} 
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken) 
\def\ep         {\ensuremath{e^+}\xspace} 
\def\epm        {\ensuremath{e^\pm}\xspace}  
\def\epem       {\ensuremath{e^+e^-}\xspace} 
\def\ee         {\ensuremath{e^-e^-}\xspace} 
 
\def\mmu        {\ensuremath{\mu}\xspace} 
\def\mup        {\ensuremath{\mu^+}\xspace} 
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken) 
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace} 
\def\mtau       {\ensuremath{\tau}\xspace} 
 
\def\taup       {\ensuremath{\tau^+}\xspace} 
\def\taum       {\ensuremath{\tau^-}\xspace} 
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace} 
 
\def\ellm       {\ensuremath{\ell^-}\xspace} 
\def\ellp       {\ensuremath{\ell^+}\xspace} 
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace} 
 
\def\nub        {\ensuremath{\overline{\nu}}\xspace} 
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace} 
\def\nub        {\ensuremath{\overline{\nu}}\xspace} 
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace} 
\def\nue        {\ensuremath{\nu_e}\xspace} 
\def\nueb       {\ensuremath{\nub_e}\xspace} 
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace} 
\def\num        {\ensuremath{\nu_\mu}\xspace} 
\def\numb       {\ensuremath{\nub_\mu}\xspace} 
\def\numnumb    {\ensuremath{\num\numb}\xspace} 
\def\nut        {\ensuremath{\nu_\tau}\xspace} 
\def\nutb       {\ensuremath{\nub_\tau}\xspace} 
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace} 
\def\nul        {\ensuremath{\nu_\ell}\xspace} 
\def\nulb       {\ensuremath{\nub_\ell}\xspace} 
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace} 
 
 
\def\g     {\ensuremath{\gamma}\xspace} 
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >> 
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace} 
 
\def\ega    {\ensuremath{e\gamma}\xspace} 
\def\game   {\ensuremath{\gamma e^-}\xspace} 
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace} 
 
 
\def\H      {\ensuremath{H^0}\xspace} 
\def\Hp     {\ensuremath{H^+}\xspace} 
\def\Hm     {\ensuremath{H^-}\xspace} 
\def\Hpm    {\ensuremath{H^\pm}\xspace} 
\def\W      {\ensuremath{W}\xspace} 
\def\Wp     {\ensuremath{W^+}\xspace} 
\def\Wm     {\ensuremath{W^-}\xspace} 
\def\Wpm    {\ensuremath{W^\pm}\xspace} 
\def\Z      {\ensuremath{Z^0}\xspace} 
 
 
\def\q     {\ensuremath{q}\xspace} 
\def\qbar  {\ensuremath{\overline q}\xspace} 
\def\qqbar {\ensuremath{q\overline q}\xspace} 
\def\u     {\ensuremath{u}\xspace} 
\def\ubar  {\ensuremath{\overline u}\xspace} 
\def\uubar {\ensuremath{u\overline u}\xspace} 
\def\d     {\ensuremath{d}\xspace} 
\def\dbar  {\ensuremath{\overline d}\xspace} 
\def\ddbar {\ensuremath{d\overline d}\xspace} 
\def\s     {\ensuremath{s}\xspace} 
\def\sbar  {\ensuremath{\overline s}\xspace} 
\def\ssbar {\ensuremath{s\overline s}\xspace} 
\def\c     {\ensuremath{c}\xspace} 
\def\cbar  {\ensuremath{\overline c}\xspace} 
\def\ccbar {\ensuremath{c\overline c}\xspace} 
\def\b     {\ensuremath{b}\xspace} 
\def\bbar  {\ensuremath{\overline b}\xspace} 
\def\bbbar {\ensuremath{b\overline b}\xspace} 
\def\t     {\ensuremath{t}\xspace} 
\def\tbar  {\ensuremath{\overline t}\xspace} 
\def\tbar  {\ensuremath{\overline t}\xspace} 
\def\ttbar {\ensuremath{t\overline t}\xspace} 
 
 
 
\def\piz   {\ensuremath{\pi^0}\xspace} 
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace} 
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace} 
\def\pip   {\ensuremath{\pi^+}\xspace} 
\def\pim   {\ensuremath{\pi^-}\xspace} 
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace} 
\def\pipm  {\ensuremath{\pi^\pm}\xspace} 
\def\pimp  {\ensuremath{\pi^\mp}\xspace} 
 
\def\kaon  {\ensuremath{K}\xspace} 
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace} 
\def\Kb    {\ensuremath{\Kbar}\xspace} 
\def\Kz    {\ensuremath{K^0}\xspace} 
\def\Kzb   {\ensuremath{\Kbar^0}\xspace} 
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace} 
\def\Kp    {\ensuremath{K^+}\xspace} 
\def\Km    {\ensuremath{K^-}\xspace} 
\def\Kpm   {\ensuremath{K^\pm}\xspace} 
\def\Kmp   {\ensuremath{K^\mp}\xspace} 
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace} 
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace}  
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace}  
\def\Kstarz  {\ensuremath{K^{*0}}\xspace} 
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace} 
\def\Kstar   {\ensuremath{K^*}\xspace} 
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace} 
\def\Kstarp  {\ensuremath{K^{*+}}\xspace} 
\def\Kstarm  {\ensuremath{K^{*-}}\xspace} 
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace} 
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace} 
 
\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace} 
 
 
 
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace} 
\def\Db      {\ensuremath{\Dbar}\xspace} 
\def\Dz      {\ensuremath{D^0}\xspace} 
\def\Dzb     {\ensuremath{\Dbar^0}\xspace} 
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace} 
\def\Dp      {\ensuremath{D^+}\xspace} 
\def\Dm      {\ensuremath{D^-}\xspace} 
\def\Dpm     {\ensuremath{D^\pm}\xspace} 
\def\Dmp     {\ensuremath{D^\mp}\xspace} 
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace} 
\def\Dstar   {\ensuremath{D^*}\xspace} 
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace} 
\def\Dstarz  {\ensuremath{D^{*0}}\xspace} 
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace} 
\def\Dstarp  {\ensuremath{D^{*+}}\xspace} 
\def\Dstarm  {\ensuremath{D^{*-}}\xspace} 
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace} 
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace} 
\def\Ds      {\ensuremath{D^+_s}\xspace} 
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace} 
\def\Dss     {\ensuremath{D^{*+}_s}\xspace} 
 
% Obsolete 
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace} 
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace} 
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace} 
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace} 
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace} 
 
 
\def\B       {\ensuremath{B}\xspace} 
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace} 
\def\Bb      {\ensuremath{\Bbar}\xspace} 
\def\BB      {\ensuremath{B\Bbar}\xspace}  
\def\Bz      {\ensuremath{B^0}\xspace} 
\def\Bzb     {\ensuremath{\Bbar^0}\xspace} 
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace} 
\def\Bu      {\ensuremath{B^+}\xspace} 
\def\Bub     {\ensuremath{B^-}\xspace} 
\def\Bp      {\ensuremath{\Bu}\xspace} 
\def\Bm      {\ensuremath{\Bub}\xspace} 
\def\Bpm     {\ensuremath{B^\pm}\xspace} 
\def\Bmp     {\ensuremath{B^\mp}\xspace} 
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace} 
\def\Bs      {\ensuremath{B_s}\xspace} 
\def\Bsb     {\ensuremath{\Bbar_s}\xspace} 
 
% added by GHM on March 25, 2003 -- from Andrei Gritsan 
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace} 
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace} 
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace} 
 
 
\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace} 
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace} 
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace} 
\def\etac     {\ensuremath{\eta_c}\xspace} 
\def\chiczero {\ensuremath{\chi_{c0}}\xspace} 
\def\chicone  {\ensuremath{\chi_{c1}}\xspace} 
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace} 
\mathchardef\Upsilon="7107 
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}! 
\def\OneS  {\Y1S} 
\def\TwoS  {\Y2S} 
\def\ThreeS{\Y3S} 
\def\FourS {\Y4S} 
\def\FiveS {\Y5S} 
 
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm 
 
 
 
\def\proton      {\ensuremath{p}\xspace} 
\def\antiproton  {\ensuremath{\overline p}\xspace} 
\def\neutron     {\ensuremath{n}\xspace} 
\def\antineutron {\ensuremath{\overline n}\xspace} 
 
\mathchardef\Deltares="7101 
\mathchardef\Xi="7104 
\mathchardef\Lambda="7103 
\mathchardef\Sigma="7106 
\mathchardef\Omega="710A 
 
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace} 
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace} 
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace} 
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace} 
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace} 
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace} 
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace} 
 
\def\X {\ensuremath{X}\xspace} 
 
 
 
\def\BR         {{\ensuremath{\cal B}\xspace}} 
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace} 
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace} 
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace} 
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace} 
 
 
 
 
\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace} 
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace} 
 
 
 
\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace} 
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace} 
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace} 
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace} 
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace} 
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace} 
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace} 
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace} 
 
\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace} 
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace} 
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace} 
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace} 
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace} 
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace} 
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace} 
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace} 
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace} 
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace} 
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace} 
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace} 
 
\def\BtoDK      {\ensuremath{B \to DK}\xspace} 
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace} 
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace} 
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace} 
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace} 
 
\def\Btoetah    {\ensuremath{B \to \eta h}\xspace} 
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace} 
 
\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace} 
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace} 
 
\def\btosgam    {\ensuremath{b \to s \g}\xspace} 
\def\btodgam    {\ensuremath{b \to d \g}\xspace} 
\def\btosll     {\ensuremath{b \to s \ellell}\xspace} 
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace} 
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace} 
\def\btosglue   {\ensuremath{b \to s g}\xspace} 
 
 
 
\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace} 
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace} 
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace} 
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace} 
 
 
 
\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace} 
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace} 
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace} 
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace} 
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace} 
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace} 
 
 
 
\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace} 
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace} 
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace} 
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace} 
 
 
 
\def\ptot       {\mbox{$p$}\xspace} 
\def\pxy        {\mbox{$p_T$}\xspace} 
\def\pt         {\mbox{$p_T$}\xspace} 
\def\mes        {\mbox{$m_{\rm ES}$}\xspace} 
\def\mec        {\mbox{$m_{\rm EC}$}\xspace} 
\def\DeltaE     {\mbox{$\Delta E$}\xspace} 
 
\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace} 
 
 
 
\def\mphi       {\mbox{$\phi$}\xspace} 
\def\mtheta     {\mbox{$\theta$}\xspace} 
\def\ctheta     {\mbox{$\cos\theta$}\xspace} 
 
 
 
\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace} 
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace} 
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace} 
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace} 
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace} 
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace} 
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace} 
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace} 
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace} 
 
 
 
\def\syin {\ensuremath{^{\prime\prime}}\xspace} 
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken 
\def\ft   {\ensuremath{\rm \,ft}\xspace} 
\def\km   {\ensuremath{{\rm \,km}}\xspace} 
\def\m    {\ensuremath{{\rm \,m}}\xspace} 
\def\cm   {\ensuremath{{\rm \,cm}}\xspace} 
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace} 
\def\mm   {\ensuremath{{\rm \,mm}}\xspace} 
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace} 
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter  
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace} 
\def\nm   {\ensuremath{{\rm \,nm}}\xspace} 
\def\fm   {\ensuremath{{\rm \,fm}}\xspace} 
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer 
% 
\def\barn{\ensuremath{{\rm \,b}}\xspace} 
\def\barnhyph{\ensuremath{{\rm -b}}\xspace} 
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace} 
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace} 
\def\nb         {\ensuremath{{\rm \,nb}}\xspace} 
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace} 
\def\pb {\ensuremath{{\rm \,pb}}\xspace} 
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace} 
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace} 
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace} 
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace} 
 
 
 
\def\mus  {\ensuremath{\rm \,\mus}\xspace} 
\def\ns   {\ensuremath{\rm \,ns}\xspace} 
\def\ps   {\ensuremath{\rm \,ps}\xspace} 
\def\fs   {\ensuremath{\rm \,fs}\xspace} 
\def\gm   {\ensuremath{\rm \,g}\xspace} 
 
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19 
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond 
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond 
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond 
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond 
 
 
 
\def\Xrad {\ensuremath{X_0}\xspace} 
\def\NIL{\ensuremath{\lambda_{int}}\xspace} 
\let\dgr\degrees 
 
 
\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace} 
 
 
\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace} 
\def\krad {\ensuremath{\rm \,krad}\xspace} 
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace} 
\def\yr   {\ensuremath{\rm \,yr}\xspace} 
\def\hr   {\ensuremath{\rm \,hr}\xspace} 
\def\degc {\ensuremath{^\circ}{C}\xspace} 
\def\degk {\ensuremath {\rm K}\xspace} 
\def\degrees{\ensuremath{^{\circ}}\xspace} 
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian 
\def\rad{\ensuremath{\rm \,rad}\xspace} 
\def\mradhyph{\ensuremath{\rm -mr}\xspace} 
% 
\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}    
\def\sz    {\ensuremath{\sigma_z}\xspace}     
 
 
% Some more (from Helen) 
\def\order{{\ensuremath{\cal O}}\xspace} 
\def\L{{\ensuremath{\cal L}}\xspace} 
\def\calL{{\ensuremath{\cal L}}\xspace} 
\def\calS{{\ensuremath{\cal S}}\xspace} 
\def\calA{{\ensuremath{\cal A}}\xspace} 
\def\calD{{\ensuremath{\cal D}}\xspace} 
\def\calR{{\ensuremath{\cal R}}\xspace} 
 
\def\ra                 {\ensuremath{\rightarrow}\xspace} 
\def\to                 {\ensuremath{\rightarrow}\xspace} 
 
 
\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace} 
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace} 
 
 
\def\pep2{PEP-II} 
\def\BF{$B$ Factory} 
\def\abf {asymmetric \BF} 
\def\sx    {\ensuremath{\sigma_x}\xspace}      
\def\sy    {\ensuremath{\sigma_y}\xspace}    
\def\sz    {\ensuremath{\sigma_z}\xspace} 
 
 
\newcommand{\inverse}{\ensuremath{^{-1}}\xspace} 
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace} 
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace} 
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace} 
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace} 
 
\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em 
          \lower.35em\hbox{$\sim$}~}\xspace} 
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em 
          \lower.35em\hbox{$\sim$}~}\xspace} 
 
\def\qsq                {\ensuremath{q^2}\xspace} 
 
 
% Data processing 
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace} 
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace} 
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace} 
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace} 
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace} 
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace} 
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace} 
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace} 
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace} 
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace} 
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace} 
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace} 
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace} 
% 
 
 
 
 
% QCD parameters 
 
\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace} 
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace} 
\newcommand{\LMSb}{% 
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace 
} 
 
% Electroweak parameters 
 
\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace} 
\newcommand{\twb}{% 
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace 
} 
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace} 
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace} 
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace} 
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace} 
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace} 
 
 
% CKM, CP violation 
 
\def\eps{\varepsilon\xspace} 
\def\epsK{\varepsilon_K\xspace} 
\def\epsB{\varepsilon_B\xspace} 
\def\epsp{\varepsilon^\prime_K\xspace} 
 
\def\CP                {\ensuremath{C\!P}\xspace} 
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \! 
% added by GHM on March 25, 2003 
\def\C       {\ensuremath{C}\xspace} 
\def\P       {\ensuremath{P}\xspace} 
\def\T       {\ensuremath{T}\xspace} 
 
 
 
\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}\xspace} 
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace} 
 
\def\rhobar {\ensuremath{\overline \rho}\xspace} 
\def\etabar {\ensuremath{\overline \eta}\xspace} 
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|,  
|\varepsilon_K|, \Delta m_{B_d}}\xspace} 
 
\def\Vud  {\ensuremath{|V_{ud}|}\xspace} 
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace} 
\def\Vtd  {\ensuremath{|V_{td}|}\xspace} 
\def\Vus  {\ensuremath{|V_{us}|}\xspace} 
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace} 
\def\Vts  {\ensuremath{|V_{ts}|}\xspace} 
\def\Vub  {\ensuremath{|V_{ub}|}\xspace} 
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace} 
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace} 
 
 
% added by Gautier for tagging, tagmix, and sin2beta 
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace} 
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace} 
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace} 
\def\mistag{\ensuremath{w}\xspace} 
\def\dilution{\ensuremath{\cal D}\xspace} 
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace} 
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace} 
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace} 
 
\newcommand{\fsubd}{\ensuremath{f_D}}\xspace 
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace} 
\newcommand{\fsubb}{\ensuremath{f_B}\xspace} 
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace} 
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace} 
\newcommand{\bsubb}{\ensuremath{B_B}\xspace} 
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace} 
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace} 
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace} 
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace} 
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace} 
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace} 
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace} 
 
\newcommand{\secref}[1]{Section~\ref{sec:#1}} 
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}} 
\newcommand{\figref}[1]{Figure~\ref{fig:#1}} 
\newcommand{\tabref}[1]{Table~\ref{tab:#1}} 
 
 
 
 
% Journal References 
 
% These bases are useful for ``submitted to'' when no volume is needed 
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace} 
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace} 
\newcommand{\jprBase}        {Phys.\ Rev.\xspace} 
\newcommand{\jplBase}        {Phys.\ Lett.\xspace} 
% update the following based on input from John Ripka, Asst. Editor at PRL, August 2006 
\newcommand{\nimBaseA}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ A\xspace} 
\newcommand{\nimBaseB}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ B\xspace} 
\newcommand{\nimBaseC}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ C\xspace} 
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ D\xspace} 
\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ E\xspace} 
\newcommand{\npBase}         {Nucl.\ Phys.\xspace} 
\newcommand{\zpBase}         {Z.\ Phys.\xspace} 
 
 
\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}} 
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}} 
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}} 
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}} 
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}} 
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}} 
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}} 
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}} 
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}} 
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}} 
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}} 
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}} 
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}} 
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}} 
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}} 
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}} 
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}} 
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}} 
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}} 
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}} 
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}} 
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}} 
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}} 
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}} 
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}} 
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}} 
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}} 
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}} 
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}} 
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}} 
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}} 
 
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}} 
\newcommand{\nimaa}       [1]  {\nimBaseE~{\bf #1}} 
\newcommand{\nima}      [1]  {\nimBaseA~{\bf #1}} 
\newcommand{\nimb}      [1]  {\nimBaseB~{\bf #1}} 
\newcommand{\nimc}      [1]  {\nimBaseC~{\bf #1}} 
\newcommand{\nimd}      [1]  {\nimBaseD~{\bf #1}} 
\newcommand{\nime}      [1]  {\nimBaseE~{\bf #1}} 
% add commands for NIM articles from earlier periods 
% for NIM articles from 1981-1983 
\newcommand{\oldnim}    [1]  {Nucl.\ Instrum.\ Methods Phys.\ Res.~{\bf #1}} 
% for NIM articles prior to 1981 
\newcommand{\oldernim}  [1]  {Nucl.\ Instrum.\ Methods~{\bf #1}} 
 
\newcommand{\np}        [1]  {\npBase\ {\bf #1}} 
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}} 
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}} 
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}} 
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}} 
 
\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}} 
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}} 
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}} 
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}} 
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}} 
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}} 
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}} 
 
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}} 
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}} 
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}} 
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}} 
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}} 
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}} 
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}} 
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}} 
 
\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}} 
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}} 
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\bf #1}}} 
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}} 
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm 
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}} 
\newcommand{\sci}       [1]  {{Science~{\bf #1}}} 
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}} 
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}} 
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}} 
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}} 
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}} 
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}} 
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}} 
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}} 
 
\newcommand{\hepex}     [1]  {hep-ex/{#1}} 
\newcommand{\hepph}     [1]  {hep-ph/{#1}} 
\newcommand{\hepth}     [1]  {hep-th/{#1}} 
 
 
\def\aslund     {\mbox{\tt Aslund}\xspace} 
\def\bbsim      {\mbox{\tt BBsim}\xspace} 
\def\beast      {\mbox{\tt Beast}\xspace} 
\def\beget      {\mbox{\tt Beget}\xspace} 
\def\Bta        {\mbox{\tt Beta}\xspace} 
\def\betakfit   {\mbox{\tt BetaKfit}\xspace} 
\def\cornelius  {\mbox{\tt Cornelius}\xspace} 
\def\evtgen     {\mbox{\tt EvtGen}\xspace} 
\def\euclid     {\mbox{\tt Euclid}\xspace} 
\def\fitver     {\mbox{\tt FitVer}\xspace} 
\def\fluka      {\mbox{\tt Fluka}\xspace} 
\def\fortran    {\mbox{\tt Fortran}\xspace} 
\def\gcalor     {\mbox{\tt GCalor}\xspace} 
\def\geant      {\mbox{\tt GEANT}\xspace} 
\def\gheisha    {\mbox{\tt Gheisha}\xspace} 
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace} 
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace} 
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace} 
\def\koralb     {\mbox{\tt KoralB}\xspace} 
\def\minuit     {\mbox{\tt Minuit}\xspace} 
\def\objegs     {\mbox{\tt Objegs}\xspace} 
\def\paw        {\mbox{\tt Paw}\xspace} 
\def\Root       {\mbox{\tt Root}\xspace} 
\def\squaw      {\mbox{\tt Squaw}\xspace} 
\def\stdhep     {\mbox{\tt StdHep}\xspace} 
\def\trackerr   {\mbox{\tt TrackErr}\xspace} 
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace} 

